Multi-variable LSTM neural network for autoregressive exogenous model

In this paper, we propose multi-variable LSTM capable of accurate forecasting and variable importance interpretation for time series with exogenous variables. Current attention mechanism in recurrent neural networks mostly focuses on the temporal aspect of data and falls short of characterizing variable importance. To this end, the multi-variable LSTM equipped with tensorized hidden states is developed to learn hidden states for individual variables, which give rise to our mixture temporal and variable attention. Based on such attention mechanism, we infer and quantify variable importance. Extensive experiments using real datasets with Granger-causality test and the synthetic dataset with ground truth demonstrate the prediction performance and interpretability of multi-variable LSTM in comparison to a variety of baselines. It exhibits the prospect of multi-variable LSTM as an end-to-end framework for both forecasting and knowledge discovery.

==> bayesnn.tex <==
Leveraging Crowdsourcing Data For Deep Active Learning
An Application: Learning Intents in Alexa

DALC adopts the Bayesian approach to deep learning recently
developed by Gal and Ghahramani [15]. Specifically, we consider a
generic DL model with parameters W as a likelihood function:
p(yi
|xi
,W) = softmax(f W(xi)) (1)
with f W(xi) modeling the output of the network layers preceding
the softmax layer. To formulate the DL model in a Bayesian
framework, we first define a prior over the parameters W:
W ∼ p(W |K) (2)
e.g., a standard Gaussian prior parameterized by K (the co-variance
matrix). With this assumption, model training will result in a posterior
distribution over the parameters, i.e., p(W|Dt r ain), instead
of point estimates, i.e., fixed values for the parameters. Note that
here we assume that the true labels are given in the training data
Dt r ain = (X, Y). We explain in Section 4 how to infer the true
labels from the observed data samples and noisy annotations.
Training & Prediction with Bayesian DL. In the following, we
describe how to train the Bayesian DL model and make predictions
with the trained model. These will be the building blocks in training
the overall DALC framework, as we will show in Section 4.
Training the Bayesian DL model is exactly similar to training a
normal DL model using the back-propagation method with dropout
enabled. The prediction given an arbitrary input x can be described
as a likelihood function:
p(y |x, Dt r ain) =
∫
p(y |x, W)p(W |Dt r ain)dW (3)
which provides a more robust prediction than non-Bayesian method
as it considers the uncertainty of the learned parameters.
The problem of inferring the exact posterior distribution for the
parameters, p(W|Dt r ain), is almost always infeasible in Bayesian


methods. Gal and Ghahramani [15] propose Monte Carlo (MC)
dropout, which is a simple yet effective method for performing
approximate variational inference. MC dropout is based on dropout
[21, 37], which is a widely used method in training DL models to
prevent over-fitting. It is generally used during the model training
process by randomly dropping hidden units of the network
in each iteration. Gal and Ghahramani [15] prove that by simply
performing dropout during the forward pass in making predictions,
the output is equivalent to the prediction when the parameters
are sampled from a variational distribution of the true posterior.
To give the intuition, the reason for the above is that test dropout
gives us predictions from different versions of the network, which
is equivalent to taking samples from a stochastic version of the
network. Uncertainty can then be estimated based on the samples
similarly to the Query by Committee [35] principle, which looks at
the degree of disagreement.
Formally, MC dropout is equivalent to sampling from a variational
distribution q(W) that minimizes the Kullback-Leibler (KL)
divergence to the true posterior p(W|Dt r ain). Given this, we can
then perform a Monte Carlo integration to approximate Equation 3:
p(y |x, Dt r ain) ≈ ∫
p(y |x, W)q(W)dW
≈
1
T
ÕT
t=1
p(y |x, W) c
(4)
where Wc is sampled T times from q(W), i.e., W ∼ c q(W). To
summarize, MC dropout provides a practical way to approximately
sample from the true posterior without explicitly calculating the
intractable true posterior.

==> model_backup.tex <==
\section{Multi-variable LSTM}


Can an RNN discover such hierarchical multiscale structure without explicit hierarchical boundary
information?


In this section, we present the proposed multi-variable LSTM referred to as MV-LSTM in detail. 
% \tao{should we include a figure for multi-variable LSTM? we can consider to shorten the introduction.}

$A^\mathsf{T}$


Assume we have $N-1$ exogenous time series and target series $\mathbf{y}$ of length $T$, where $\mathbf{y} = ( y_1, \cdots, y_T )$ and $\mathbf{y} \in \mathbb{R}^T$.\footnote{
Vectors are assumed to be in column form throughout this paper.
} 
By stacking exogenous time series and target series, we define the multi-variable input of MV-LSTM at each time step as
$\mathbf{X} = ( \mathbf{x}_1, \ldots, \mathbf{x}_T )$, 
where $ \mathbf{x}_t = ( x_{t,1}, \ldots, x_{t, N-1}, y_{t} )  \in \mathbb{R}^N$ is the multi-variable input at time step $t$ and $x_{t,n} \in \mathbb{R}$ is the observation of $n$-th exogenous time series at time $t$.
% each dimension corresponds to the observations of a variable. since each hidden state ingest information from all input variable, has to develop seperated rnn to individual model 
Given $\mathbf{X}$, we aim to learn a non-linear mapping to the one-step ahead value of the target series, namely $\hat{y}_{T+1} = \mathcal{F}(\mathbf{X})$,
where $\mathcal{F}(\cdot)$ represents the MV-LSTM neural network we present below. 

% kaiser2017depthwise, kuchaiev2017factorization, 
Inspired by \citet{he2017wider}, our MV-LSTM has tensorized hidden states and the update scheme ensures that each element of the hidden state tensor encapsulates information exclusively from a certain variable of the input.
% , while it is updated by exploiting multi-variable input together.

Specifically, we define the hidden state and memory cell for $t$-th time step of MV-LSTM as 
$\mathbf{h}_t \in \mathbb{R}^M$ and $\mathbf{c}_t \in \mathbb{R}^M$, 
where $M$ is the size of recurrent layer. 
$\mathbf{h}_t$ is tensorized as 
$\mathcal{H}_t = [ \mathbf{h}_t^{1}, \ldots, \mathbf{h}_t^{N} ]^\top $, 
where $\mathcal{H}_t \in \mathbb{R}^{N \times d}$, $\mathbf{h}_t^{n} \in \mathbb{R}^d$ and $N \cdot d = M$. 
The element $\mathbf{h}_t^{n}$ of tensor $\mathcal{H}_t$ is a variable specific representation corresponding to $n$-th input dimension.
% as well as evolving correlatively. 
% The update process in MV-LSTM presented below ensures that such representations
% as the gates for updating are derived by using all input dimensions.
We further define the input-to-hidden transition tensor as 
$\mathcal{W}_x = [ \mathbf{W}_x^{1}, \ldots, \mathbf{W}_x^{N} ]^\top $, 
where $\mathcal{W}_x \in \mathbb{R}^{N \times d }$ and $\mathbf{W}_x^{n} \in \mathbb{R}^d $. 
The hidden-to-hidden transition tensor is defined as: 
$\mathcal{W}_h = [ \mathbf{W}_h^{1}, \ldots, \mathbf{W}_h^{N} ]^\top$, 
where $\mathcal{W}_h \in \mathbb{R}^{N \times d \times d}$ and 
$\mathbf{W}_h^{n} \in \mathbb{R}^{d \times d}$.

% characterised by its ability to have different recurrent transition functions for each possible input, w


\tian{tensornized temporal attention}
\tian{tensor dot}
Tensor contraction of a and b along specified axes.

Tensordot (also known as tensor contraction) sums the product of elements from a and b over the indices specified by 



Given the new incoming input $\mathbf{x}_t$ and the hidden state $\mathbf{h}_{t-1}$ up to $t-1$,
% and $\mathbf{c}_{t-1}$,
we formulate the iterative update process by using $\mathcal{W}_x$ and $\mathcal{W}_h$ as:
\begin{align*}
   \mathbf{j}_t = \tanh( \mathcal{H}_{t - 1} * \mathcal{W}_h + \mathbf{x}_t * \mathcal{W}_x + \mathbf{b}_j )&= \tanh \left( \begin{bmatrix}
           (\mathbf{W}_h^1 \mathbf{h}_{t-1}^1)^\top \\
           \vdots \\
            (\mathbf{W}_h^N \mathbf{h}_{t-1}^N)^\top 
         \end{bmatrix} 
         +
         \begin{bmatrix}
           (\mathbf{W}_x^1 x_{t, 1})^\top \\
           \vdots \\
           (\mathbf{W}_x^N x_{t, N})^\top
         \end{bmatrix} 
         + \mathbf{b}_j \right)
\end{align*} 
where $*$ represents the element-wise multiplication operation on tensor elements. 
$\mathcal{H}_{t-1} * \mathcal{W}_h \in \mathbb{R}^{N \times d}$ 
is the concatenation of $N$ product results of hidden tensor element $\mathbf{h}_t^{n}$
and the corresponding transition matrix $\mathbf{W}_h^{n}$. 
Likewise, 
% the result of 
$ \mathbf{x}_t * \mathcal{W}_x \in \mathbb{R}^{N \times d}$,
% is a $M$ dimensional vector, 
and represents how the current input $\mathbf{x}_t$ update the hidden state. 

$\mathbf{j}_t$ is an $N \times d$ dimensional tensor, and each $d$-dimensional element corresponds to one input variable, 
% as well as encoding information exclusively from that variable. 
encoding the information exclusively from the variable specific hidden state and the input variable.
% Therefore, elements in $\mathbf{j}_t$ can be grouped the same way as tensorized $\mathcal{H}_t$, each of which corresponds to a certain variable. 
% Different from the tensorized update of $\mathbf{j}_t$,

The input, forget and output gates in MV-LSTM are updated by using all input dimensions of $\mathbf{x}_t$, so as to utilize the cross-correlation between multi-variable time series. 

In particular, 

$[\mathbf{i}_t, \mathbf{f}_t, \mathbf{o}_t]^{\top} = \sigma \left( \mathbf{W}  [\mathbf{x}_t, \mathbf{h}_{t-1}] + \mathbf{b} \right)$.
% \begin{align}
% \begin{bmatrix}
% \mathbf{i}_t \\
% \mathbf{f}_t \\
% \mathbf{o}_t \\
% \end{bmatrix}
% &= \sigma \left( \mathbf{W}  [\mathbf{x}_t, \mathbf{h}_{t-1}] + \mathbf{b} \right) 
% \end{align} 
The updated memory cell and hidden states are obtained from 

$\mathbf{c}_t = \mathbf{f}_t \odot \mathbf{c}_t + \mathbf{i}_t \odot \mathbf{\tilde{j}}_t $,

where $\mathbf{\tilde{j}}_t \in \mathbb{R}^M $ is the flattened vector of $\mathbf{j}_t$. Then, $\mathbf{h}_t = \mathbf{o}_t \odot \tanh(\mathbf{c}_t)$.


After feeding $\mathbf{x}_T$ into MV-LSTM, 
we obtain the hidden representation $\mathbf{h}_T^n$ w.r.t. each variable, which can be combined with the attention mechanism to predict $y_{T+1}$ 
as well as interpreting variable importance. 





Concretely, the attention process is as: 

$e^n = \tanh( \mathbf{W}_e \mathbf{h}_{T}^n + b_e )$ and $\alpha^n = \frac{exp(e^n)}{\sum_{k=1}^N exp(e^k)}$. 

Then, the prediction is derived as: 

$\hat{y}_{T+1} = \sum_{n=1}^N \alpha^n ( \mathbf{W_n} \mathbf{h}_n^{\top} + b_n )$.

Note that MV-LSTM is able to apply temporal attention with ease. In the present work, we focus on evaluating variable attention. 

% \tian{loss function}

% Wider and Deeper, Cheaper and Faster: Tensorized LSTMs for Sequence Learning
% Tensorizing Neural Networks
% FACTORIZATION TRICKS FOR LSTM NETWORKS
